Requirements-driven Test Generation for Autonomous Vehicles with Machine Learning Components

Autonomous vehicles are complex systems that are challenging to test and debug. A requirements-driven approach to the development process can decrease the resources required to design and test these systems, while simultaneously increasing the reliability. We present a testing framework that uses signal temporal logic (STL), which is a precise and unambiguous requirements language. Our framework evaluates test cases against the STL formulae and additionally uses the requirements to automatically identify test cases that fail to satisfy the requirements. One of the key features of our tool is the support for machine learning (ML) components in the system design, such as deep neural networks. The framework allows evaluation of the control algorithms, including the ML components, and it also includes models of CCD camera, lidar, and radar sensors, as well as the vehicle environment. We use multiple methods to generate test cases, including covering arrays, which is an efficient method to search discrete variable spaces. The resulting test cases can be used to debug the controller design by identifying controller behaviors that do not satisfy requirements. The test cases can also enhance the testing phase of development by identifying critical corner cases that correspond to the limits of the system's allowed behaviors. We present STL requirements for an autonomous vehicle system, which capture both component-level and system-level behaviors. Additionally, we present three driving scenarios and demonstrate how our requirements-driven testing framework can be used to identify critical system behaviors, which can be used to support the development process.

==> exp_results.tex <==
\subsection{Experiment Results}

We applied the testing strategies described in Sec. \ref{sec:strategies} to $\modeld$.
Fig. \ref{fig:probability_distribution} illustrates how the glancing-case robustness values fit to a truncated normal distribution for different test approaches, together with the mean robustness values.
The robustness values closer to zero represent a better performance for the related test approach, as they correspond to behaviors where a collision either nearly occurred or nearly did not occur.
For each test approach we perform 20 trials, each with a total budget of 200 simulations.


%Table \ref{table:exp_results} provides the results.
%For each strategy the average of worst-case and glancing case robustness results over several trials are provided.
%For the worst-case robustness values (``Average Worst-case Robustness''), more negative numbers are better, as they indicate that a more severe collision was identified.
%Alternatively, for the glancing case robustness (``Average Glancing-case robustness''), values closer to $0$ are better, as they correspond to behaviors where a collision either nearly occurred or nearly did not occur.

%The column ``Average Worst-case Robustness'' presents the average of the found worst-case Robustness values with each test approach.
%The column ``Average Glancing-case robustness'' presents the average of the found \textit{close-to-zero} robustness values with each test approach.
%Smaller values indicate better performance.

 
For \GUR, the average robustness values reported are the mean of the robustness values with minimum absolute value over the 20 trials.

%is the uniform random search over the discrete and continuous parameters.
%We have executed 7 Global UR tests, each with a budget of 200 simulations.

%The second and third row of the table present the results for the \CAUR and \CASA tests.
For the \CAUR and \CASA approaches, we first generate a 2-way covering array: $CA(2, 16, (v_1, ..., v_{16}))$ where $v_1, ..., v_{16}$ are each the number of possible discrete values a parameter can take.
The number of possible values is $v_1 = ... = v_5 = 5$ for the colors of the vehicles, $v_6 = ... = v_{10} = 5$ for the models of the vehicles, $v_{11}, v_{12} = 5$ for the Jay-walking Pedestrian shirt and pants colors, $v_{13} = 2$ for the existence (True/False) of fog, $v_{14} = 4$ for the discretized space of the Ego vehicle position, $v_{15} = 4$ for the discretized space of the agent Vehicle 1 position, and $v_{16} = 4$ for the discretized space of the Pedestrian speed.
The size of that covering array is 47, and it covers all possible $2,562$ 2-way combinations, while the number of all possible combinations of all parameters would be $5^{12}\cdot 2 \cdot 4^3$.

%If we WLOG, the covering array strength can be increased beyond 2, with the cost of executing more simulations.

Each of the \CAUR and \CASA runs begins with the 47 covering array test cases (i.e., these runs account for 47 of the 200 simulations allotted to each trial).
Then, for the test cases that have the closest robustness value to their target (robustness values closest to $0$), the search continues over the real-valued space for 153 additional simulations.
Hence, each \CAUR and \CASA trial has a total budget of 200 simulations, which is equal to the simulation budget for each \GUR trial.
Also, for the \CAUR and \CASA test cases, we limit the maximum number of search iterations (simulations) starting from a given discrete case ($\pd_{d_j}$) to 50, 
at which time we restart the search at the \emph{next best} discrete case and perform another search; this repeats until the total simulation budget of 200 is spent.
For \CAUR and \CASA, as we target finding a glancing case (close to zero robustness value), we take the absolute value of the robustness.
%For each covering array test case, we further limit the maximum number of simulations by 50 for a falsification attempt.
%For \CAUR and \CASA we do 2 separate runs, one is with the target of finding a worst-case (minimum robustness value) failure, the other is with the target of finding a glancing case (close to zero robustness value).

Fig. \ref{fig:probability_distribution} shows that, compared to the \GUR method, the \CAUR method does a better job of identifying glancing cases and also has the advantage of guaranteeing that any 2-way combination among the parameters are covered in our search space, while still using an unguided approach to explore the real-valued space.
%Thus, the improved performance for the worst-case search is expected, but the poor performance for the glancing case is not; we attribute the decline in performance for the glancing case to a statistical aberration. 
\begin{figure}[b]
	\vspace*{-0.15in}
	\centering
	\includegraphics[width=0.6\linewidth]{figures/exp_result_plot.pdf}
	\vspace*{-0.05in}
	\caption{Probability distribution of the robustness values.}
	\label{fig:probability_distribution}
	%\vspace*{-0.2in}
\end{figure}

The \CASA method does better than both the \GUR and \CAUR method in identifying glancing behaviors.
As can be seen in Fig. \ref{fig:probability_distribution}, \CASA, on average, can find the test cases that generate a behavior closer to the target (i.e., close to $0$).
The \CASA approach, while maintaining the coverage guarantees inherited from covering arrays, also applies falsification in the continuous space, and so \CASA is expected to perform better than either of the other two methods. 
The results in Fig. \ref{fig:probability_distribution} confirm this analysis.
%Fig. \ref{fig:probability_distribution} illustrates how the glancing-case robustness values fit to a normal distribution for different test approaches.
%As it can be seen in the figure, with \CASA, the expected robustness value is closer to zero with a smaller variance, which shows its advantage in searching for a corner-case compared to the other methods.
%\begin{table}[htb] 
%	\centering  
%	\caption{Evaluation results for autonomous driving testing framework. } \label{table:exp_results}  
%	\begin{tabular}{|c|K{3cm}|K{3.5cm}|}\hline
%		Test Type & Average Worst-case Robustness & Average Glancing-case Robustness\\
%		\hline
%		\GUR & -16.46 & 1.91 \\
%		\CAUR & -18.91 & 1.45 \\
%		\CASA & -16.33 & 0.54 \\
%		\hline
%	\end{tabular}
%\end{table} 


We believe that these results indicate that an approach combining covering arrays and optimization-based falsification, such as \CASA, can be useful in testing autonomous driving systems, especially if specific combinations of some discrete parameters that cannot be directly discovered by intuition may generate challenging scenarios for perception systems.
%, which are critical for object detection and classification.

\iffalse 

Fig. \ref{fig:covering_array_failing_nonfailing} illustrates the importance of discrete parameter combinations selected by the covering array.
Fig. \ref{fig:covering_array_failing_nonfailing}a shows a failing test case from the covering array.
Fig. \ref{fig:covering_array_failing_nonfailing}b presents the same example with only the modification we have manually made on the color of the vehicle 4, which results in a non failing test case.
\begin{figure}[htp]
	\vspace*{-0.2in}
	\begin{center}
		\begin{tabular}{c}
			\includegraphics[width=.24\textwidth]{figures/s_a_1.png}\hspace{0in}
			\includegraphics[width=.24\textwidth]{figures/s_a_2.png}\hspace{0in}
			\includegraphics[width=.24\textwidth]{figures/s_a_3.png}\hspace{0in}
			\includegraphics[width=.24\textwidth]{figures/s_a_4.png}\\
			(a)\vspace{0in} \\
			\includegraphics[width=.24\textwidth]{figures/s_b_1.png}\hspace{0in}
			\includegraphics[width=.24\textwidth]{figures/s_b_2.png}\hspace{0in}
			\includegraphics[width=.24\textwidth]{figures/s_b_3.png}\hspace{0in}
			\includegraphics[width=.24\textwidth]{figures/s_b_4.png}\\
			(b)\\
		\end{tabular}
		\vspace*{-0.1in}
		\caption{Chronologically ordered images from (a) a failing test from the covering array and (b) a non-failing test after only changing the color of a vehicle.}
		\label{fig:covering_array_failing_nonfailing}
	\end{center}
	\vspace*{-0.2in}
\end{figure}

\fi

%\begin{figure}[htp]
%	\centering
%	\includegraphics[width=.24\textwidth]{figures/s_a_1.png}\hfill
%	\includegraphics[width=.24\textwidth]{figures/s_a_2.png}\hfill
%	\includegraphics[width=.24\textwidth]{figures/s_a_3.png}\hfill
%	\includegraphics[width=.24\textwidth]{figures/s_a_4.png}
%	\caption{Chronologically ordered images from a failing test from the covering array}
%	\label{fig:covering_array_failing}
%\end{figure}
%\begin{figure}[htp]
%	\centering
%	\includegraphics[width=.24\textwidth]{figures/s_b_1.png}\hfill
%	\includegraphics[width=.24\textwidth]{figures/s_b_2.png}\hfill
%	\includegraphics[width=.24\textwidth]{figures/s_b_3.png}\hfill
%	\includegraphics[width=.24\textwidth]{figures/s_b_4.png}
%	\caption{Chronologically ordered images from a non-failing test by only changing the color of a vehicle}
%	\label{fig:covering_array_nonfailing}
%\end{figure}



==> figures/FrameworkFlowchart_discrete.tex <==
\begin{tikzpicture}[>=stealth',scale=0.6, every node/.style={scale=0.6}]

\tikzset{
  font={\fontsize{14pt}{14}\selectfont}}

\tikzstyle{stext}=[font=\fontsize{14}{14}\selectfont]
\tikzstyle{smalltext}=[font=\fontsize{14}{14}\selectfont]
\tikzstyle{block}=[draw,fill=white,rectangle,minimum height=2em,text
                   width=4.5em,fill=blue!10,stext,inner sep=4pt,align=center,execute at begin node=\setlength{\baselineskip}{1.2em}]
\tikzstyle{file}=[tape,fill=red!10,tape bend top=none,draw,inner
                  sep=2pt,text width=5em,align=center,smalltext,execute at begin node=\setlength{\baselineskip}{1.2em}]
\tikzstyle{note} = [coordinate]

\node[file, fill=green!20, text width=6em]  (discrete init) {};
\node[block, below of=discrete init, node distance=14mm, text width=18em] (combinatorial) {\textsc{Combinatorial Test Gen.}};
\draw[->] (discrete init) -- node[name=discrete space, right, text width=12em,execute at begin node=\setlength{\baselineskip}{1.2em}] {Discrete Space} (combinatorial);

\node[block, below left=1.5em and -18mm of combinatorial, text width=11em] (sim int discrete) {\textsc{Sim. Interface}};
\draw[->] (combinatorial) -- node[name=setup discrete, left, text width=7em,execute at begin node=\setlength{\baselineskip}{1.2em}] {Test Setup} (sim int discrete);

\node[stext, below right=6mm and -8mm of combinatorial, text width=1em] (s1) {\textsc{.}};
\draw[->] (combinatorial) -- node[name=setup discrete 2, left, text width=7em,execute at begin node=\setlength{\baselineskip}{1.2em}] { } (s1);
\node[stext, below of=s1, node distance=5.4mm, text width=1em] (s3) {\textsc{.}};
\node[stext, below of=s3, node distance=5.4mm, text width=1em] (s4) {\textsc{.}};
\node[stext, below of=s4, node distance=5.4mm, text width=1em] (s5) {\textsc{.}};
\node[stext, below of=s5, node distance=5.4mm, text width=1em] (s6) {\textsc{.}};
\node[stext, below of=s6, node distance=5.4mm, text width=1em] (s7) {\textsc{.}};
\node[stext, below of=s7, node distance=5.4mm, text width=1em] (s11) {\textsc{.}};

\node[stext, right of=s1, node distance=12mm, text width=1em] (s2) {\textsc{.}};
\draw[->] (combinatorial) -- node[name=setup discrete 2, left, text width=7em,execute at begin node=\setlength{\baselineskip}{1.2em}] { } (s2);
\node[stext, below of=s2, node distance=5.4mm, text width=1em] (s3) {\textsc{.}};
\node[stext, below of=s3, node distance=5.4mm, text width=1em] (s4) {\textsc{.}};
\node[stext, below of=s4, node distance=5.4mm, text width=1em] (s5) {\textsc{.}};
\node[stext, below of=s5, node distance=5.4mm, text width=1em] (s6) {\textsc{.}};
\node[stext, below of=s6, node distance=5.4mm, text width=1em] (s7) {\textsc{.}};
\node[stext, below of=s7, node distance=5.4mm, text width=1em] (s12) {\textsc{.}};

\node[block, below of=sim int discrete, node distance=16mm, text width=13em] (sim env discrete) {\textsc{Sim. Environment}};
\draw[->] (sim int discrete) -- node[name=setup discrete, right, text width=16em,execute at begin node=\setlength{\baselineskip}{1.2em}] {Scenario} (sim env discrete);

\node[block, below of=sim env discrete, node distance=16mm, text width=11em] (cost discrete) {\textsc{Cost Function}};
\draw[->] (sim env discrete) -- node[name=simresults discrete, right]{Sim. Trace} (cost discrete);

\node[block, below of=combinatorial, node distance=64mm, text width=17em] (minimum discrete) {\textsc{Extract Best Test Case}};
\draw[->] (cost discrete) -- node[name=simresults discrete, right]{\ Cost} (minimum discrete);
\draw[->] (s11) -- node[name=simresults discrete, right]{} (minimum discrete);
\draw[->] (s12) -- node[name=simresults discrete, right]{} (minimum discrete);

\node[draw, rounded corners ,align=center, below of=minimum discrete, node distance=16mm,fill=red!10,text width=6em] (stop discrete) {\textsc{Halt}};
\draw[->] (minimum discrete) -- node[name=best result discrete, right]{Best Test Setup} (stop discrete);

\end{tikzpicture}

==> figures/FrameworkFlowchart_falsify.tex <==
\begin{tikzpicture}[>=stealth',scale=0.6, every node/.style={scale=0.6}]

\tikzset{
  font={\fontsize{14pt}{14}\selectfont}}

\tikzstyle{stext}=[font=\fontsize{14}{14}\selectfont]
\tikzstyle{smalltext}=[font=\fontsize{14}{14}\selectfont]
\tikzstyle{block}=[draw,fill=white,rectangle,minimum height=2em,text
                   width=4.5em,fill=blue!10,stext,inner sep=4pt,align=center,execute at begin node=\setlength{\baselineskip}{1.2em}]
\tikzstyle{file}=[tape,fill=red!10,tape bend top=none,draw,inner
                  sep=2pt,text width=5em,align=center,smalltext,execute at begin node=\setlength{\baselineskip}{1.2em}]
\tikzstyle{note} = [coordinate]

\node[file,fill=green!20, text width=6em]  (init setup) {};

\node[block,below of= init setup, node distance=18mm, text width=9em] (sim int) {\textsc{Simulation \\Interface}};

\node[block,below of=sim int, node distance=22mm, text width=10em] (s) {\textsc{Simulation \\Environment}};

\node[block,below of=s,node distance=21mm,text width=11em] (cost) {\textsc{Cost Function}};

\node[draw,smalltext,diamond,aspect=2,text width=5em,below of=cost,fill=yellow!10,node distance=18mm,inner sep=0pt,align=center] (decision) 
     {$c<0$?};

\node[block,below of=decision,node distance=18mm,text width=12em] (optim) {\textsc{Optimization}};

\node[draw,rounded corners,align=center, right of= decision, node distance=32mm,fill=red!10,text width=6em] (stop) 
     {\textsc{Halt}};
\node [note,name=bugfound, font=\Large, below right=0.4cm and -0.5cm of stop,label={Bug found!}] {};

\draw[->] (init setup) -- node[name=initalize, right, text width=9em,execute at begin node=\setlength{\baselineskip}{1.2em}] {Initial Setup} (sim int);

\draw[->] (sim int) -- node[name=initalize, right, text width=5em,execute at begin node=\setlength{\baselineskip}{1.2em}] {Scenario} (s);

\draw[->] (s) -- node[name=simresults, right]{Simulation Trace} (cost);

\draw[->] (cost) -- node[name=costout, right]{c} (decision);

\draw[->] (decision) -- node[name=no,right]{No} (optim);

\draw[->] (decision) -- node[name=yes,above, near start]{Yes} (stop);

\draw [->] (optim.west) -| node[name=newparam, left, near end, text width=3em,execute at begin node=\setlength{\baselineskip}{1.2em}]{} ($(sim int.west)+(-2.0,0.0)$) -- (sim int.west) ;
\end{tikzpicture}

==> figures/FrameworkOverview.tex <==
\begin{tikzpicture}[auto, node distance=5cm,>=latex',scale=0.4, every node/.style={scale=0.4}]

\tikzset{
  font={\fontsize{18pt}{18}\selectfont}}

% Define Styles
\tikzstyle{block} = [draw, font=\Large, fill=green!20, rectangle, 
    minimum height=4em, minimum width=6em,align=center,execute at begin node=\setlength{\baselineskip}{1.5em}]
\tikzstyle{texts} = [minimum height=4em, minimum 	width=6em,align=center,execute at begin node=\setlength{\baselineskip}{1.5em}]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
%\draw[help lines] (-2,-2) grid (10,7);
    
    % We start by placing the blocks
    \node [draw, rectangle, rounded corners=5pt, minimum width=21.2cm, minimum height=7.5cm, fill=black!10,label={[anchor=north west, inner sep=10pt]north west:Simulation Environment}] (sim env) at (7.75,0.75) {};
    
	\node [draw, rectangle, rounded corners=5pt, minimum width=9.5cm, minimum height=4.5cm, fill=blue!10,label={[anchor=north west, inner sep=10pt]north west:Webots}] (webots) at (12.5,0.75) {};    
    
	\node [draw, rectangle, rounded corners=5pt, minimum width=5cm, minimum height=4.5cm, fill=blue!10,label={[anchor=north west, inner sep=10pt]north west:Tensorflow}] (tensorflow) at (0.5,0.75) {};

	\node [draw, rectangle, rounded corners=5pt, minimum width=4cm, minimum height=3cm, fill=red!10,label={[anchor=north west, inner sep=10pt]north west:SqueezeDet}] (squeezedet) at (0.55,0.25) {};

    \node [block,xshift=0.5cm,text width=9em](perception){\textsc{Perception System}} ;
    
    \node [block,right of=perception,text width=10em] (controller) {\textsc{Controller}};

  \node [block,right of=controller,xshift=0.05cm,text width=12em] (environment) {\textsc{Vehicle and Environment Model}};

\node [block,right of=environment, xshift=-0.5cm,text width=8em] (renderer) {\textsc{Renderer}};
  

%\node [texts,name=nextlabel,above of=python,node distance=4cm,align=left,text width=6em] {Python};
    
 \draw [very thick,->] (perception) --  node [name=r] {}(controller);
  \draw [very thick,->] (controller) -- node [name=m] {} (environment);
   \draw [very thick,->] (environment) -- node [name=out] {} (renderer);
  
   
\draw [very thick,->] ($(renderer.east)$) -- ($(renderer.east)+(1.25,0)$) -- ($(renderer.east)+(1.25,-2.5)$) -| (perception.south) ;

\end{tikzpicture}



==> stl_specs_for_experiments.tex <==

\subsection{STL Specifications} \label{sec:stl_specs_for_experiments}
Below is the STL specification used in our experiments:
\vspace*{-0.09in}
\begin{align*}
\phid =& \Box (\pi_{v_{ego}, mov.}\hspace{-0.04in} \implies\hspace{-0.04in} (\neg \pi_{0, coll} \wedge ... \wedge \neg\pi_{l, coll} \wedge \\
&\neg\pi_{0, \overline{coll}} \wedge ... \wedge \neg\pi_{l, \overline{coll}}))\\
\text{where, }\forall i \in &\{1, .., l\},\\
\pi_{v_{ego}, mov.} = & v_{ego} > \epsilon_{speed}\\
\pi_{i, coll} = & dist(i, ego) < \epsilon_{dist} \wedge \textit{front}(i, ego) = \top\\
\pi_{i, \overline{coll}} = & dist(i, ego) < 0
\end{align*}

In the above specification, the Ego vehicle is indexed with $ego$, and all other objects in the environment are indexed from $1$ to $l$.
Position of an object is represented with $\mathbf{x}$.
$\textit{front}(i, ego)$ evaluates to true ($\top$) if object $i$ is partially in the front corridor of the Ego vehicle and to false ($\bot$) otherwise.
$\textit{dist}(i, ego)$ gives the minimum Euclidean distance between front bumper of the Ego vehicle and the object $i$.
The specification basically describes that the Ego vehicle should not hit another vehicle or pedestrian.
The predicates $\pi_{i, \overline{coll}}, \forall i \in \{1, ..., l\}$ are added so that the robustness corresponds to the  Euclidean distance of the corresponding object when it is not in front corridor of the Ego vehicle.
